Template Controllable keywords-to-text Generation

This paper proposes a novel neural model for the understudied task of generating text from keywords. The model takes as input a set of un-ordered keywords, and part-of-speech (POS) based template instructions. This makes it ideal for surface realization in any NLG setup. The framework is based on the encode-attend-decode paradigm, where keywords and templates are encoded first, and the decoder judiciously attends over the contexts derived from the encoded keywords and templates to generate the sentences. Training exploits weak supervision, as the model trains on a large amount of labeled data with keywords and POS based templates prepared through completely automatic means. Qualitative and quantitative performance analyses on publicly available test-data in various domains reveal our system's superiority over baselines, built using state-of-the-art neural machine translation and controllable transfer techniques. Our approach is indifferent to the order of input keywords.

==> 03_central_idea.tex <==
\section{Central Idea}
\label{sec:central}
%Most languages provide large number of ways for constructing sentences to convey the same meaning. However, structures within a language are often repetitive and can be largely covered by a finite set of syntactic and stylistic variations. For example, the way humans greet each other can be captured through a limited number of recurring greeting styles. 
Modern language generators (especially the neural models) are over-burdened due to the fact that they have to learn syntax from sparse sentences in the training data, apart from learning to filter content from the input. Generators could really benefit if they do not have to learn and infer syntax. They may rather receive syntax specifications from the user in the form of recurring templates at run-time, where templates can be either formed by the user or derived from exemplar sentences. This forms the basis of our approach. 

%A \textit{data-to-text} generator should ideally not worry about the syntax - this is why rule driven traditional NLG methods were quite effective \cite{reiter2000building}. It should rather focus on how to: (a) extract relevant content from the input keywords and determine the order in which the selected context should appear in the output, and (b) logically derive appropriate morphological forms of the content words and also intermittently introduce function words as necessary. We contend that these processes can be made smoother by guiding the generator (in our  case, a neural decoder) with the help of a template (\textit{i.e.,} POS tag sequence of an exemplar sentence).

Our framework considers a set of keywords as input supplemented with a POS tag sequence as template. Additionally, it also considers the universal POS forms of the keywords. Keywords and the templates are encoded into vector forms following standard neural encoding techniques. The decoder, however, unlike traditional decoders \cite{BahdanauCB14}, is forced to generate a finite number of words, same as the number of POS units in the template. During generation, based on the POS representation, the decoder shifts its focus between keyword representations, and generic POS representations. This helps it to decide whether to: (a) produce a word related to the input keywords and in what morphological form, or (b) introduce a function word (\textit{e.g.} preposition) based on the POS and previously generated words. 

The key advantages of using such a system are:
\begin{itemize}
     \item The burden of learning deep syntactic structures in a language is less due to the additional template input which is easy to provide.
    \item Since POS tag sequences are chosen as input, they provide additional hints about the morphological, lexical and syntactic changes to be made to the keywords and what function-words to be additionally used.
    \item Out of a few possible POS tags (such as NOUNs, VERBs, \textit{etc.}), a large number of POS categories can map to only a few candidate words in the vocabulary. This significantly limits the number of choices for a large number of decoding steps.
\end{itemize}
In the following section, we describe our system in detail. 


==> 07_discussion.tex <==
\section{Discussion}
\label{sec:discussion}
